GuidedSampling: Steering LLMs Towards Diverse Candidate Solutions at Inference-Time

Repeated Sampling (RS) is a simple inference-time algorithm that has been shown to improve model performance on complex tasks. Although it is an effective way of scaling inference time, it often struggles to generate diverse solution candidates, frequently relying on the same underlying approach to solve the problem and thus producing redundant samples. To address this limitation, we propose a new inference algorithm, GuidedSampling, which decouples the exploration and generation phases during inference, increasing diversity of generated candidate solutions. The exploration phase identifies multiple concepts that can be utilized to solve the problem, while the generation phase applies a specific concept to provide final solution candidates. We first define the theoretical bounds of GuidedSampling and then empirically demonstrate that it improves the performance of base model at pass@50 by on an average ~21.6% across various benchmarks compared to RS. Furthermore, models trained on trajectories of GuidedSampling exhibit substantial performance improvements at pass@5 by on an average ~9.7%, compared to models trained on traditional RS. Additionally, models trained with GuidedSampling increases the average number of concepts per instance (1.67 -> 3.03), yielding a diverse set of candidates than traditional RS.

==> sections/sec_4_inference_aware.tex <==



\input{tables/bonbon}



==> tables/bonbon.tex <==



\begin{table*}[ht]
\footnotesize
\centering
\begin{tabular}{@{}c|c|c|c|c|c|c@{}}
\toprule
Method                        & \multicolumn{2}{c|}{MATH}           & \multicolumn{2}{c|}{GPQA-Diamond}   & \multicolumn{2}{c}{HumanEval}       \\
\cmidrule(l){2-7}
                              & pass@1           & pass@10          & pass@1           & pass@10          & pass@1           & pass@10          \\
\midrule
Base Model                    & 24.00\%          & 38.40\%          & 11.62\%          & 33.84\%          & 27.44\%          & 45.73\%          \\
BoNBoN                        & \%               & \%               & \%               & \%               & \%               & \%               \\
\midrule
\textsc{GuidedSampling}  &                  &                  &                  &                  &                  &                  \\
\multicolumn{1}{l|}{\quad + FA ; Same Concept}  & \% & \% & \% & \% & \% & \% \\
\multicolumn{1}{l|}{\quad + FA ; Diff Concept}  & \% & \% & \% & \% & \% & \% \\
\multicolumn{1}{l|}{\quad + IAA ; Same Concept} & \% & \% & \% & \% & \% & \% \\
\multicolumn{1}{l|}{\quad + IAA ; Diff Concept} & \% & \% & \% & \% & \% & \% \\
\bottomrule
\end{tabular}
\caption{Performance of Llama-3.2-3B-Instruct trained using inference-aware algorithm. FA: Just using the final answer for training the model. IAA: Using both the ideas and the corresponding final solution to create the final data. Same Idea: Responses are sampled from the same concept. Diff Idea: Responses are sampled from different concepts.}
\label{table:bonbon}
\end{table*}




% \begin{table}[ht]
%   \footnotesize
%   \centering
%   \begin{tabularx}{\linewidth}{>{\raggedright\arraybackslash}X|c|c|c|c|c|c}
%     \toprule
%     \thead{Build \\ Method} &
%     \thead{Validation \\ Successes} &
%     \thead{Total Binaries} &
%     \thead{Binary Functions} \\
%     \midrule
%     GHCC                                          & 48  & 118 & 29,063  \\
%     Assemblage                                    & 16  & 92  & 22,729  \\
%     Zero‑shot LLM (o3‑mini)                       & 9   & 34  & 14,711  \\
%     Zero‑shot LLM (Claude 3.7‑Sonnet)             & 37  & 359 & 88,692 \\ 
%     \midrule
%     Agentic Compilation (o3‑mini)                 & 112 & \textbf{1,516} & \textbf{564,235}  \\
%     \quad + Agentic Retrieval (o3‑mini)           & 104 & 848 & 436,974 \\
%     \quad + LLM‑assisted Retrieval (o3‑mini)      & 115 & 1,358 & 484,062 \\
%     \quad \textbf{+ LLM‑assisted Retrieval (Claude 3.7‑Sonnet)} & \textbf{127} & 1,316 & 490,284 \\
%     \bottomrule
%   \end{tabularx}
%   \label{tab: binary dataset stats}
% \end{table}
